Arma: Byzantine Fault Tolerant consensus with Linear Scalability

Arma is a Byzantine Fault Tolerant (BFT) consensus system designed to achieve linear scalability across all hardware resources: network bandwidth, CPU, and disk I/O. As opposed to preceding BFT protocols, Arma separates the dissemination and validation of client transactions from the consensus process, restricting the latter to totally ordering only metadata of batches of transactions. This separation enables each party to distribute compute and storage resources for transaction validation, dissemination and disk I/O among multiple machines, resulting in linear scalability. Additionally, Arma ensures censorship resistance by imposing a maximum time limit for the inclusion of client transactions. We build a prototype implementation of Arma and evaluate its performance experimentally. Our results show that Arma totally orders over 100,000 transactions per second when deployed in a WAN setting and integrated into Hyperledger Fabric.

==> patch <==
diff --git a/ARMA.tex b/ARMA.tex
index f515550..4823246 100644
--- a/ARMA.tex
+++ b/ARMA.tex
@@ -432,8 +432,9 @@ making transaction validation and routing horizontally scalable.
 
 \subsubsection{Mapping transactions to shards}
 
- To ensure censorship resistance and de-duplication, the function that maps transactions to shards must be deterministic. In this way, all parties' routers would forward the received transactions to the appropriate batchers, ensuring that all batchers within the shard will receive the transaction. Additionally,
-for effective load balancing, the router must distribute the transactions
+To ensure censorship resistance and de-duplication, it is essential that transactions are mapped to shards in a deterministic manner. 
+In this way, assuming a client follows the protocol, and submits the transaction to all parties, all honest parties' routers would  forward the received transactions to the appropriate batchers, ensuring that all honest batchers of the shard will receive the transaction. 
+Additionally, for effective load balancing across the shards, the router must distribute the transactions
 among the known $k$ shards in a manner that is as close to a uniform distribution
 across the set $\left\{ 1,..,k\right\} $ as possible.
 
@@ -444,7 +445,8 @@ like a CRC checksum can be employed without compromising its functionality.
 
 
 \subsubsection{Transaction verification}
-Besides forwarding transactions to their corresponding shards, router nodes also ensure only transactions that are well formed and properly signed by clients are forwarded. In earlier protocols such as \cite{Mir-BFT}, each party ran a single node which was involved in verifying all transactions arriving from clients to that party. In Arma, however, a party can utilize the router nodes to horizontally scale the CPU intensive task of verifying signatures and offload it from the batcher nodes. Identifying ineligible transactions and excluding them from the next steps, ensure that system resources are properly devoted to the processing of correctly formed transactions. 
+
+Besides forwarding transactions to their corresponding shards, routers also ensure only transactions that are well formed and properly signed by clients are forwarded. In earlier protocols such as \cite{Mir-BFT}, each party ran a single node which was involved in verifying all transactions arriving from clients to that party. In Arma, however, a party can utilize the routers to horizontally scale the CPU intensive task of verifying signatures and alleviating the batcher nodes. Identifying ineligible transactions and excluding them from the next steps, ensure that system resources are properly devoted to the processing of correctly formed transactions. 
 
 
 \subsection{Transaction Batching}

